Evaluating LLM-driven User-Intent Formalization for Verification-Aware Languages

Verification-aware programming languages such as Dafny and F* provide means to formally specify and prove properties of a program. Although the problem of checking an implementation against a specification can be defined mechanically, there is no algorithmic way of ensuring the correctness of the {\it user-intent formalization for programs}, expressed as a formal specification. This is because intent or requirement is expressed {\it informally} in natural language and the specification is a formal artefact. Despite, the advent of large language models (LLMs) has made tremendous strides bridging the gap between informal intent and formal program implementations recently, driven in large parts by benchmarks and automated metrics for evaluation. Recent work has proposed a framework for evaluating the {\it user-intent formalization} problem for mainstream programming languages~\cite{endres-fse24}. However, such an approach does not readily extend to verification-aware languages that support rich specifications (using quantifiers and ghost variables) that cannot be evaluated through dynamic execution. Previous work also required generating program mutants using LLMs to create the benchmark. We advocate an alternate, perhaps simpler approach of {\it symbolically testing specifications} to provide an intuitive metric for evaluating the quality of specifications for verification-aware languages. We demonstrate that our automated metric agrees closely on a human-labeled dataset of Dafny specifications for the popular MBPP code-generation benchmark, yet demonstrates cases where the human labeling is not perfect. We also outline formal verification challenges that need to be addressed to apply the technique more widely. We believe our work provides a stepping stone to enable the establishment of a benchmark and research agenda for the problem of user-intent formalization for programs.

==> evalspec.tex <==
\section{Metrics for evaluating a specification}
\label{sec:problem}

We would like to design a metric that has the following desirable properties:
\begin{enumerate}
    \item The metric should be objective, and should not vary by user.
    \item The metric should be evaluated automatically without any manual effort.
    \item The metrics should reward a precise specification with a score close to 1, and should penalize an incorrect specification with lowest score 0. But it should reward specifications that are correct yet precise proportional to its discriminative power to distinguish incorrect implementations.
\end{enumerate}

In this section, we first describe our metrics for any verification-aware language. Then we present our implementation for Dafny language. 

\subsection{Proposal: Testing specifications}

Consider a method with signature \code{m(x):y} denoting the name \code{m}, input parameters \code{x} and output parameters \code{y}, a candidate postcondition/summary specification $\spec{}$(\code{x}, \code{y}) and a set of input-output tests $\tests{}$.

\subsubsection{Correctness}
A postcondition $\spec{}$(\code{x}, \code{y}) is correct (or sound) with respect to $\tests{}$ if it is consistent with all the input-output pairs in $\tests{}$.
In other words, for each $(i, o) \in \tests{}$ the following Hoare-triple~\cite{hoare} holds.
$$
\models \{\btrue\} \ \code{x} := i; \ \code{y} := o; \ \{\spec{}(\code{x}, \code{y})\}
$$

\subsubsection{Completeness}
The completeness measure for a specification $\spec{}$ given   $\tests{}$ is the fraction of output mutations of the tests in $\tests{}$ that $\spec{}$ is inconsistent with.
Let $\tests{1} \doteq \bigcup_{(i,o) \in \tests{}} \bigcup_{o' \neq o} \{(i,o')\}$ be a finite set of mutations of $\tests{}$.
In this work, we restrict the set of mutants per input $i$ to a fixed number (5 for this paper).
Let $\tests{2} \subseteq \tests{1}$ be the largest subset such that for each $(i,o') \in \tests{2}$, the following Hoare-triple does not hold:
$$
\not\models \{\btrue\} \ \code{x} := i; \ \code{y} := o'; \ \{\spec{}(\code{x}, \code{y})\}
$$
Then the completeness measure of $\spec{}$ with respect to $\tests{}$ is $|\tests{2}|/|\tests{1}|$.
This is inspired by the work on {\it mutation-testing} literature~\cite{mutation-testing-cite} where the completeness measure is similar to the {\it kill-set} denoting the number of input-output mutants that can be distinguished by the specification.

\subsection{Alternate proposal}
A reader may wonder if the following check achieves a similar objective:
$$
\models \{\code{x} == i \wedge \spec{}(\code{x}, \code{y})\} \ \code{skip} \ \{\code{y} == o\}
$$
There are two issues with this formulation: (a) this only provides a Boolean metric that only rewards a precise specification that constrains \code{y} to a unique value $o$. For example, it would award the strong (yet imprecise) specifications of \code{SharedElements} to 0. Secondly, (b) this formulation is also too strong when the precise functional specification allows for non-determinism in the output. Consider the running example of \code{SharedElements}, where the specification allows for the output to be one of either $\{[4, 5], [5, 4]\}$ for the given inputs.


==> fmcad.old.tex <==
\NeedsTeXFormat{LaTeX2e}
\ProvidesClass{fmcad}[FMCAD class]

% Author: Georg Weissenbacher
% Copyright FMCAD Association (CC BY-SA)
% ORCID Logo: ORCID (2017) https://doi.org/10.23640/07243.5008697.v2
% CC-BY Logo from https://creativecommons.org/about/downloads/
% doi logo from commons.wikimedia.org

% This package is to be used in combination with
% IEEEtran.cls (c) by Michael Shell a under LaTeX Project Public License 
\LoadClass[conference]{IEEEtran}

% The options of the following packages might clash with
% packages loaded later, e.g., \usepackage[table]{xcolor}
% will lead to a clash. This can be avoided by adding
% \PassOptionsToPackage{table}{xcolor} _before_
% \documentclass{fmcad}

%%
%% We declare the options doi, startpage, and pdfa
%% 
\RequirePackage{ifthen}
\RequirePackage{kvoptions}
\SetupKeyvalOptions{
  family=fmcad,
  prefix=fmcad@
}
\DeclareStringOption[]{doi}
\DeclareStringOption[]{startpage}
\DeclareStringOption[21]{year}

\newboolean{fmcad@mkpdfa}
\setboolean{fmcad@mkpdfa}{false}
\DeclareVoidOption{pdfa}{\setboolean{fmcad@mkpdfa}{true}}

\ProcessKeyvalOptions*\relax

\PassOptionsToPackage{hyperref}{hidelinks}

% check whether user wants to generate PDF/A
\iffmcad@mkpdfa
\RequirePackage[a-1b]{pdfx}
\fi

\RequirePackage{hyperref}
\hypersetup{hidelinks}

\RequirePackage{tikz}
\usetikzlibrary{svg.path}



%%
%% Define colors
%%
\definecolor{fmcadblue}{HTML}{2C3E6B}
\definecolor{orcidgreen}{HTML}{A6CE39}
\definecolor{ccbygray}{HTML}{AAB2AB}
\definecolor{doiorange}{HTML}{FCB425}

%%
%% Define new heades and footers
%%

\pagestyle{headings}

% if startpage is defined then show page numbers, else don't
\ifthenelse{\equal{\fmcad@startpage}{}}{}
           {\pagenumbering{arabic}\setcounter{page}{\fmcad@startpage}}
\newcommand{\fmcad@thepage}{
  \ifthenelse{\equal{\fmcad@startpage}{}}{}{\thepage}}

% Link to ORCID
\newcommand\orcid[1]{\href{https://orcid.org/#1}{\raisebox{-.15em}{\resizebox{1em}{1em}{%
      \begin{pgfpicture}
        \pgfsetcolor{orcidgreen}
        \pgfpathsvg{M106.301,35.435c0,19.572-15.863,35.436-35.436,35.436S35.43,55.007,35.43,35.435S51.293,0,70.865,0
	S106.301,15.863,106.301,35.435z}
        \pgfusepath{fill}
        \pgfsetcolor{white}
        \pgfpathsvg{M59.321,32.39v13.398h-4.264V16.14h4.264V32.39z}
        \pgfpathsvg{M65.578,16.112h11.572c9.772,0,15.724,7.226,15.724,14.839c0,7.004-4.816,14.838-15.779,14.838H65.578 V16.112z M69.841,41.941h6.562c8.305,0,12.098-5.039,12.098-10.99c0-3.654-2.215-10.99-11.877-10.99h-6.782V41.941z}
        \pgfpathsvg{M57.189,54.758c-1.55,0-2.796-1.245-2.796-2.796c0-1.523,1.246-2.797,2.796-2.797s2.796,1.273,2.796,2.797 C59.985,53.485,58.74,54.758,57.189,54.758z}
        \pgfusepath{fill}
      \end{pgfpicture}%
  }}}}

% FMCAD symbol
\newcommand\fmcadsymbol{
  \begin{pgfpicture}
    \pgfsetcolor{fmcadblue}
    \pgfpathsvg{M23.801,12.698c0.282,0,0.537,0.115,0.723,0.3c0.186,0.186,0.301,0.44,0.302,0.721h-0.002 c0,0.283-0.115,0.537-0.3,0.723c-0.187,0.186-0.442,0.303-0.723,0.303V14.74c-0.282,0-0.536-0.113-0.722-0.299 c-0.185-0.186-0.3-0.439-0.3-0.721h-0.002c0.001-0.282,0.116-0.537,0.302-0.723S23.52,12.698,23.801,12.698L23.801,12.698z M20.898,22.705c0.278,0,0.533,0.115,0.72,0.301s0.301,0.441,0.301,0.722h-0.002c0,0.282-0.113,0.537-0.299,0.722 c-0.186,0.186-0.441,0.299-0.722,0.299h-0.001v0.002c-0.28,0-0.536-0.115-0.722-0.301c-0.185-0.185-0.299-0.439-0.299-0.721v-0.001 h-0.002c0.001-0.28,0.114-0.536,0.301-0.722s0.442-0.301,0.722-0.301l0.001,0.002l0,0L20.898,22.705z M7.234,18.349 c0.281,0,0.536,0.115,0.721,0.3c0.186,0.185,0.301,0.44,0.301,0.722H8.254c0,0.281-0.114,0.536-0.299,0.721 c-0.185,0.186-0.439,0.3-0.72,0.302H7.231c-0.28-0.002-0.534-0.116-0.719-0.302c-0.186-0.185-0.3-0.439-0.3-0.721v-0.002 l-0.002,0.002c0-0.281,0.115-0.537,0.302-0.722C6.696,18.464,6.951,18.349,7.234,18.349L7.234,18.349 M18.896,32.585L32.32,19.16 v-5.599L18.76,0h-5.386l-1.767,1.767l1.996,1.996l-0.425,0.426l2.294,2.293l2.062,0.024c0.123-0.431,0.351-0.813,0.658-1.118 c0.469-0.47,1.117-0.759,1.834-0.759l0.002-0.004c0.718,0,1.367,0.291,1.837,0.762c0.469,0.468,0.759,1.117,0.759,1.835 l0.003,0.001v0.001l-0.003,0.002c0,0.717-0.29,1.366-0.759,1.834c-0.47,0.471-1.119,0.761-1.837,0.761l-0.002-0.002 c-0.718,0-1.365-0.29-1.835-0.759c-0.272-0.272-0.485-0.606-0.615-0.979L15.129,8.05c-0.214-0.002-0.405-0.09-0.546-0.229 l-0.001,0.001l-2.519-2.518l-0.4,0.4L9.666,3.708L8.893,4.481l1.996,1.996l-0.396,0.396l6.311,6.312 c0.045-0.009,0.09-0.013,0.137-0.013l4.317,0.018c0.104-0.505,0.355-0.956,0.706-1.307c0.47-0.471,1.119-0.76,1.836-0.76h0.001 c0.717,0,1.366,0.289,1.837,0.76c0.468,0.469,0.758,1.117,0.758,1.834l0.002,0.002c0,0.718-0.29,1.367-0.76,1.837 c-0.47,0.469-1.118,0.759-1.835,0.759l-0.003,0.003c-0.717,0-1.366-0.291-1.837-0.761c-0.228-0.227-0.412-0.496-0.542-0.793 l-3.051-0.014l3.456,3.457l-0.002,0.002c0.142,0.143,0.23,0.34,0.23,0.558l-0.011,2.616v0.017c0.255,0.126,0.488,0.293,0.687,0.491 c0.469,0.469,0.759,1.117,0.759,1.835l0.004,0.002c0,0.717-0.291,1.366-0.762,1.837c-0.47,0.471-1.12,0.76-1.836,0.76h-0.001 l-0.002-0.002c-0.719,0-1.365-0.289-1.834-0.758c-0.471-0.471-0.762-1.119-0.762-1.836v-0.001l0.002-0.002 c0-0.718,0.291-1.366,0.76-1.835c0.375-0.376,0.865-0.637,1.416-0.725l0.007-2.074L9.379,7.987L8.948,8.419L6.952,6.423 L6.178,7.195l1.996,1.998L7.76,9.606l6.979,6.979l-0.002,0.002c0.145,0.145,0.234,0.346,0.229,0.567l-0.042,3.159 c0.093,0.06,0.18,0.129,0.261,0.21c0.613,0.615,0.613,1.613,0,2.227c-0.615,0.616-1.613,0.616-2.229,0 c-0.616-0.613-0.616-1.611,0-2.227c0.119-0.12,0.253-0.216,0.396-0.289l0.038-2.766l-6.746-6.746l-0.412,0.412L4.237,9.137 L3.464,9.912l1.996,1.994L5.006,12.36l3.062,3.062l-0.001,0.002c0.137,0.138,0.225,0.326,0.229,0.537l0.025,1.051 c0.28,0.129,0.533,0.307,0.749,0.523c0.468,0.467,0.758,1.116,0.758,1.834l0.003,0.002c0,0.717-0.291,1.366-0.761,1.836 c-0.469,0.469-1.118,0.758-1.835,0.758H7.231c-0.717,0-1.366-0.289-1.834-0.758c-0.472-0.47-0.762-1.119-0.762-1.836v-0.002h0.003 c0-0.718,0.29-1.367,0.759-1.834c0.359-0.361,0.825-0.615,1.346-0.716l-0.012-0.503l-2.84-2.84l-0.372,0.371l-1.996-1.996L0,13.375 v5.662l13.548,13.549H18.896z M20.028,6.203c0.283,0,0.537,0.113,0.723,0.299s0.299,0.44,0.301,0.721v0.001H21.05v0.001h0.002 v0.002c-0.002,0.281-0.115,0.533-0.301,0.72c-0.186,0.185-0.44,0.3-0.723,0.3v0.002c-0.281,0-0.535-0.115-0.722-0.302 c-0.185-0.185-0.3-0.44-0.3-0.722l-0.002-0.002c0-0.28,0.115-0.534,0.302-0.721c0.187-0.186,0.442-0.301,0.722-0.301V6.203z}
    \pgfusepath{fill}
  \end{pgfpicture}
}

% CC BY logo
\newcommand\ccbylogo{
  \begin{pgfpicture}
    \pgfsetcolor{ccbygray}
    \pgfpathsvg{M179.087,38.513V0.807h119.82l0.14,37.567c0,3.416-1.423,3.18-3.017,3.18l-114.064,0.202 C179.25,41.757,179.087,40.198,179.087,38.513z}
    \pgfusepath{fill}
    \pgfsetcolor{black}
    \pgfpathsvg{M299.558,40.007V0.51c0-0.282-0.229-0.51-0.511-0.51h-119.73c-0.282,0-0.51,0.228-0.51,0.51v39.497 c0,1.246,1.015,2.26,2.261,2.26h116.229C298.544,42.268,299.558,41.253,299.558,40.007z M179.828,40.007c0,0,0-15.949,0-27.45 h4.078c3.043-5.509,8.908-9.244,15.643-9.244c6.732,0,12.599,3.739,15.644,9.244h83.344c0,11.502,0,27.45,0,27.45 c0,0.683-0.556,1.238-1.24,1.238H181.067C180.384,41.245,179.828,40.69,179.828,40.007z}
    \pgfusepath{fill}
    \pgfsetcolor{white}
    \pgfpathsvg{M253.077,9.311h-3.141V2.648h3.236c0.3,0,0.591,0.037,0.875,0.112s0.537,0.19,0.758,0.346 c0.221,0.155,0.398,0.356,0.529,0.601s0.197,0.537,0.197,0.873c0,0.417-0.102,0.774-0.305,1.069 c-0.203,0.297-0.511,0.503-0.924,0.621c0.299,0.143,0.526,0.326,0.678,0.551c0.153,0.223,0.23,0.502,0.23,0.838 c0,0.313-0.052,0.572-0.154,0.784c-0.103,0.211-0.249,0.381-0.435,0.508c-0.187,0.128-0.411,0.219-0.672,0.275 C253.684,9.283,253.396,9.311,253.077,9.311L253.077,9.311z M251.405,6.616v1.555h1.374c0.13,0,0.257-0.011,0.378-0.032 c0.121-0.021,0.229-0.06,0.322-0.116c0.093-0.056,0.168-0.134,0.225-0.233c0.055-0.099,0.084-0.227,0.084-0.382 c0-0.279-0.084-0.481-0.253-0.604c-0.169-0.124-0.383-0.187-0.645-0.187H251.405z M251.405,3.788v1.828h1.6 c0.317,0,0.573-0.073,0.766-0.218c0.193-0.146,0.29-0.391,0.29-0.733c0-0.173-0.029-0.316-0.089-0.428 c-0.059-0.112-0.138-0.2-0.238-0.265c-0.1-0.065-0.216-0.112-0.346-0.141c-0.132-0.028-0.268-0.042-0.412-0.042H251.405z}
    \pgfpathsvg{M258.234,5.242V2.648h1.469v2.557l2.473,4.106h-1.633l-1.551-2.632l-1.561,2.632h-1.644 L258.234,5.242z}
    \pgfusepath{fill}
    \pgfsetcolor{white}
    \pgfpathsvg{M213.774,23.091c-0.006,7.972-6.469,14.428-14.44,14.424 c-7.971-0.007-14.429-6.472-14.424-14.44c0-0.006,0-0.013,0-0.018c0.004-7.969,6.471-14.426,14.44-14.422 c7.971,0.006,14.427,6.47,14.422,14.44C213.774,23.079,213.774,23.085,213.774,23.091z}
    \pgfusepath{fill};
    \pgfsetcolor{black}
    \pgfpathsvg{M199.322,39.629c-4.58,0-8.455-1.6-11.627-4.801c-3.257-3.311-4.885-7.229-4.885-11.754 c0-4.528,1.628-8.417,4.885-11.673c3.254-3.255,7.132-4.884,11.627-4.884c4.552,0,8.497,1.642,11.835,4.925 c3.146,3.118,4.717,6.995,4.717,11.632c0,4.634-1.6,8.553-4.8,11.754S203.957,39.629,199.322,39.629z M199.372,36.649 c3.752,0,6.949-1.317,9.584-3.954c2.636-2.636,3.955-5.846,3.955-9.627c0-3.808-1.298-6.967-3.893-9.479 c-2.732-2.705-5.949-4.058-9.647-4.058c-3.7,0-6.887,1.339-9.564,4.017c-2.678,2.676-4.017,5.851-4.017,9.52 c0,3.672,1.353,6.875,4.057,9.607C192.442,35.325,195.618,36.649,199.372,36.649z M199.157,25.806 c-0.882,1.603-2.343,2.408-4.38,2.408c-1.378,0-2.527-0.462-3.45-1.39c-0.923-0.924-1.386-2.177-1.386-3.75 c0-1.604,0.448-2.86,1.344-3.773c0.895-0.912,2.087-1.366,3.573-1.366c1.928,0,3.375,0.855,4.338,2.569l-2.021,1.077 c-0.414-0.958-1.102-1.437-2.065-1.437c-1.46,0-2.188,0.981-2.188,2.946c0,1.964,0.729,2.947,2.188,2.947 c0.826,0,1.445-0.451,1.857-1.354L199.157,25.806z M208.715,25.806c-0.878,1.603-2.336,2.408-4.371,2.408 c-1.403,0-2.559-0.462-3.464-1.39c-0.907-0.924-1.361-2.177-1.361-3.75c0-1.604,0.447-2.86,1.341-3.773 c0.895-0.912,2.083-1.366,3.567-1.366c1.925,0,3.371,0.855,4.332,2.569l-2.068,1.077c-0.385-0.958-1.062-1.437-2.025-1.437 c-1.489,0-2.233,0.981-2.233,2.946c0,1.964,0.744,2.947,2.233,2.947c0.799,0,1.407-0.451,1.819-1.354L208.715,25.806z}
    \pgfusepath{fill}
    \pgfsetcolor{white}
    \pgfpathsvg{M265.092,27.184c-0.004,5.261-4.27,9.522-9.53,9.52c-5.26-0.006-9.522-4.271-9.52-9.531 c0-0.004,0-0.008,0-0.011c0.003-5.26,4.27-9.521,9.53-9.519c5.26,0.005,9.521,4.271,9.519,9.53 C265.092,27.175,265.092,27.18,265.092,27.184z}
    \pgfusepath{fill}
    \pgfsetcolor{black}
    \pgfpathsvg{M258.678,30.081v-4.772h-1.332v-5.653h-3.617v5.653h-1.33v4.772c0,0.417,0.338,0.753,0.752,0.753h4.774 C258.34,30.834,258.678,30.498,258.678,30.081L258.678,30.081z}
    \pgfusepath{fill}
    \pgfsetcolor{black}
    \pgfpathsvg{M263.82,35.477c2.258-2.256,3.388-5.017,3.388-8.285c0-3.267-1.11-6-3.331-8.195 c-2.354-2.315-5.139-3.471-8.354-3.471c-3.174,0-5.909,1.147-8.207,3.442c-2.299,2.294-3.446,5.038-3.446,8.227 s1.149,5.951,3.446,8.285c2.24,2.256,4.975,3.383,8.207,3.383C258.795,38.859,261.561,37.732,263.82,35.477z M248.836,33.959 c-1.908-1.924-2.863-4.182-2.863-6.768s0.942-4.822,2.834-6.708c1.887-1.886,4.135-2.829,6.746-2.829 c2.609,0,4.877,0.953,6.805,2.859c1.832,1.77,2.746,3.997,2.746,6.68c0,2.664-0.935,4.92-2.804,6.767 c-1.849,1.867-4.1,2.802-6.747,2.802C252.904,36.76,250.666,35.826,248.836,33.959z}
    \pgfusepath{fill}
    \pgfsetcolor{black}
    \pgfpathsvg{M257.212,33.035c0,0.922-0.748,1.669-1.67,1.669c-0.921-0.002-1.668-0.75-1.668-1.671 c0,0,0-0.001,0-0.002c0-0.921,0.748-1.668,1.67-1.668c0.921,0,1.668,0.748,1.668,1.67C257.212,33.033,257.212,33.033,257.212,33.035 z}
    \pgfusepath{fill}
  \end{pgfpicture}
}

% DOI logo
\newcommand\doilogo{
  \begin{pgfpicture}
    \pgfsetcolor{doiorange}
    \pgfpathsvg{M128.993,65.002c0.021,35.325-28.609,63.971-63.955,64C29.695,129.02,1.018,100.4,1,65.08 c0-0.021,0-0.051,0-0.077C0.979,29.685,29.618,1.031,64.964,1.001c35.352-0.018,64.012,28.597,64.038,63.928 C129.002,64.955,129.002,64.98,128.993,65.002z}
    \pgfusepath{fill}
    \pgfsetcolor{black}
    \pgfpathsvg{M49.819,104.629H37.965v-25.42c-1.357,1.408-3.649,2.855-4.93,3.469c-2.228,1.076-5.354,1.304-7.89,1.304 c-4.353,0-8.456-2.315-11.81-5.21c-4.226-3.637-6.338-8.502-6.338-14.597c0-5.992,1.937-11.552,6.06-15.188 c3.458-3.048,7.401-4.447,11.831-4.447c2.74,0,5.661,0.783,7.812,1.986c1.229,0.691,4.061,2.232,5.265,3.743v-4.825h11.854V104.629z M34.791,57.672c-1.562-1.562-4.273-2.519-6.552-2.519c-2.535,0-4.246,1.299-5.833,3.193c-1.306,1.537-2.047,3.73-2.047,5.701 c0,1.973,0.653,4.341,1.959,5.878c1.613,1.895,3.938,3.721,6.448,3.721c2.253,0,5.14-1.408,6.728-2.996 c1.588-1.562,2.206-4.26,2.206-6.515C37.699,61.857,36.378,59.234,34.791,57.672z}
    \pgfusepath{fill}
    \pgfsetcolor{white}
    \pgfpathsvg{M110.459,102.311c1.384-1.357,2.075-3.021,2.075-4.994c0-1.996-0.691-3.688-2.075-5.07 c-1.356-1.357-3.033-2.035-5.031-2.035c-1.972,0-3.649,0.691-5.032,2.074c-1.356,1.383-2.036,3.061-2.036,5.031 c0,1.973,0.68,3.637,2.036,4.994c1.383,1.383,3.061,2.074,5.032,2.074S109.076,103.693,110.459,102.311z M74.219,84.495 c6.736,0,12.113-2.283,16.134-6.849c3.278-3.729,4.917-8.174,4.917-13.333c0-5.215-1.626-9.686-4.879-13.414 c-3.943-4.539-9.462-6.809-16.555-6.809c-7.119,0-12.651,2.27-16.595,6.809c-3.252,3.729-4.878,8.308-4.878,13.738 c0,4.89,1.639,9.226,4.917,13.009C61.249,82.212,66.896,84.495,74.219,84.495L74.219,84.495z M111.728,83.108V45.474h-12.6v37.635 H111.728z M67.459,69.946c-1.332-1.647-1.998-3.526-1.998-5.633c0-2.135,0.666-4.025,1.998-5.674c1.639-2.053,3.764-3.08,6.377-3.08 c2.33,0,4.302,0.838,5.915,2.514c1.613,1.701,2.42,3.781,2.42,6.24c0,2.431-0.819,4.483-2.458,6.159 c-1.613,1.702-3.572,2.555-5.877,2.555C71.223,73.027,69.098,72,67.459,69.946z}
    \pgfusepath{fill}
  \end{pgfpicture}
}

\makeatletter

% Add page numbers to standard page style
\def\@oddfoot{\hbox{}\footnotesize\hfil\fmcad@thepage\hfil}\relax
\def\@evenfoot{\hbox{}\footnotesize\hfil\fmcad@thepage\hfil}\relax

\def\ps@IEEEtitlepagestyle{% Override IEEE titlepage with FMCAD titlepage
  \def\@oddhead{\hbox{}\normalfont\hfil\href{https://fmcad.org/FMCAD\fmcad@year}{\raisebox{-.25em}{\resizebox{1.5em}{!}{\fmcadsymbol}} \color{black}{Formal Methods in Computer-Aided Design 20\fmcad@year}} \hfil}\relax
  \def\@oddfoot{%
    \begin{minipage}[b]{\textwidth}
      \raisebox{\baselineskip}{\rule{.25\textwidth}{.5pt}}\newline
      \href{https://doi.org/\fmcad@doi}{
        {\normalsize\raisebox{-.35em}{\resizebox{1.5em}{!}{\doilogo}}}}
        {\footnotesize \url{https://doi.org/\fmcad@doi}}%
      \hfill
      \href{https://creativecommons.org/licenses/by/4.0/}{
        \footnotesize\raisebox{-.75\baselineskip}{\resizebox{!}{2\baselineskip}{\ccbylogo}}
      \parbox{.3\textwidth}{\footnotesize 
        \color{black}{
          This article is licensed under a Creative
          \hbox{Commons} Attribution 4.0 International License}}}
      \hfill
    \end{minipage}}\relax
  \let\@evenhead\@empty
  \let\@evenfoot\@empty
}

\makeatother

% Print copyright notice to console
\AtEndDocument{
  \typeout{}
  \typeout{FMCAD document class by FMCAD Association (under a CC BY-SA license).}
  \typeout{}
}
